Export complexity, industrial complexity and regional economic growth in Brazil

Research on productive structures has shown that economic complexity conditions economic growth. However, little is known about which type of complexity, e.g., export or industrial complexity, matters more for regional economic growth in a large emerging country like Brazil. Brazil exports natural resources and agricultural goods, but a large share of the employment derives from services, non-tradables, and within-country manufacturing trade. Here, we use a large dataset on Brazil's formal labor market, including approximately 100 million workers and 581 industries, to reveal the patterns of export complexity, industrial complexity, and economic growth of 558 micro-regions between 2003 and 2019. Our results show that export complexity is more evenly spread than industrial complexity. Only a few -- mainly developed urban places -- have comparative advantages in sophisticated services. Regressions show that a region's industrial complexity is a significant predictor for 3-year growth prospects, but export complexity is not. Moreover, economic complexity in neighboring regions is significantly associated with economic growth. The results show export complexity does not appropriately depict Brazil's knowledge base and growth opportunities. Instead, promoting the sophistication of the heterogeneous regional industrial structures and development spillovers is a key to growth.

==> table1.tex <==
\begin{table}[!t]
\centering
\caption{Activities (products and industries) in the Bottom-5 and Top-5 of complexity estimated from exports (top) and industry (bottom), and the region with the highest RCA on such activity.}
\label{Table1}
\begin{tabular}{lll}
\hline
\rowcolor[HTML]{C0C0C0} 
\multicolumn{3}{l}{\cellcolor[HTML]{C0C0C0}\textbf{Product Complexity (Exports Data)}}                          \\ \hline
\rowcolor[HTML]{EFEFEF} 
product                                                      & PCI    & micro-region with highest RCA           \\ \hline
1801: Cocoa (whole or broken), raw or roasted                & -2.895 & Tomé-Açu, PA (RCA = 34.1)               \\
2609: Tin ores and concentrates                              & -2.874 & Ariquemes, RO (RCA = 1523.0)            \\
2602: Manganese ores \& concentrates inc mangnfrs iron ores  & -2.694 & Chorozinho, CE (RCA = 2680.2)           \\
2709: Crude oil from petroleum and bituminous minerals       & -2.636 & Baía da Ilha Grande, RJ (RCA = 18.2)    \\
5201: Cotton, not carded or combed                           & -2.606 & Tesouro, MT (RCA = 1270.3)              \\ \hline
...                                                          & ...    & ...                                     \\
9010: Apparatus and equipment for photographic…              & 2.094  & Barra do Piraí, RJ (RCA = 0.002)        \\
8461: Machine-tools for planing, shaping, slotting, …        & 2.104  & Itajubá, MG (RCA = 3.86)                \\
3707: Chemical preparations for photographic uses …          & 2.217  & Mogi das Cruzes, SP (RCA = 1.11)        \\
8457: Machining centres, unit construction machines …        & 2.411  & Sorocaba, SP (RCA = 3.50)               \\
3705: Photographic plates and film, exposed and …            & 2.468  & Jundiaí, SP (RCA = 2.99)                \\ \hline
\rowcolor[HTML]{C0C0C0} 
\multicolumn{3}{l}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \textbf{Industry Complexity (Industry Data)}}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
industry                                                     & ICI    & micro-region with highest RCA           \\ \hline
7227: Tin Ore Extraction                                     & -2.310 & Rio Preto da Eva, AM (RCA = 4408.5)     \\
84116: General Public Administration                         & -2.105 & Traipu, AL (RCA = 5.96)                 \\
7243: Precious Metal Ore Extraction                          & -2.056 & S. Miguel do Araguaia, GO (RCA = 228.6) \\
3213: Aquaculture in salty and brackish water                & -1.958 & Litoral Sul, RN (RCA = 403.7)           \\
47121: Retail trade of general merchandise ...               & -1.933 & Oiapoque, AP (RCA = 8.82)               \\
...                                                          & ...    & ...                                     \\
64328: Investment Banks                                      & 2.625  & São Paulo, SP (RCA = 7.57)              \\
64506: Capitalization Companies                              & 2.899  & Rio de Janeiro, RJ (RCA = 8.80)         \\
30504: Manufacturing of Military Combat Vehicles             & 3.521  & Campinas, SP (RCA = 49.54)              \\
66118: Administration of Exchanges and …                     & 3.671  & Osasco, SP (RCA = 8.92)                 \\
64409: Commercial Leasing                                    & 3.671  & Osasco, SP (RCA = 52.5)                 \\ \hline
\end{tabular}
\end{table}

==> table2.tex <==
\begin{table}[]
\centering
\caption{Top and bottom regions based on their industry-based and export-based economic complexity index in 2019. The numbers in parentheses correspond to the position in the IndECI ranking. The list only contains micro-regions that have exports (and, therefore, an ECI value)}
\label{Table2}
\begin{tabular}{lllll}
\multicolumn{2}{c}{\textbf{IndECI ranking}}                           &  & \multicolumn{2}{c}{\textbf{ECI ranking}}                           \\ \cline{1-2} \cline{4-5} 
\cellcolor[HTML]{EFEFEF}IndECI & \cellcolor[HTML]{EFEFEF}Micro-region &  & \cellcolor[HTML]{EFEFEF}ECI & \cellcolor[HTML]{EFEFEF}Micro-region \\ \cline{1-2} \cline{4-5} 
3.0496                         & (1) Osasco                           &  & 2.5853                      & (355) Codó                           \\
3.0405                         & (2) Guarulhos                        &  & 2.5256                      & (421) Propriá                        \\
3.0120                         & (3) São Paulo                        &  & 2.1786                      & (85) Santa Rita do Sapucaí           \\
2.9832                         & (4) Porto Alegre                     &  & 2.1187                      & (144) Não-Me-Toque                   \\
2.9411                         & (5) Campinas                         &  & 2.0276                      & (145) Bacia de São João              \\
...                             & ...                                   &  & ...                          & ...                                   \\
-1.5087                        & (543) Caracaraí                      &  & -3.2764                     & (513) Tesouro                        \\
-1.5386                        & (545) Boca do Acre                   &  & -3.2764                     & (273) Alto Paraguai                  \\
-1.6240                        & (547) Bico do Papagaio               &  & -3.2764                     & (317) Esperança                      \\
-1.8027                        & (551) Chapadas das Mangabeiras       &  & -3.3258                     & (157) Baía da Ilha Grande            \\
-1.9403                        & (556) Cotegipe                       &  & -3.4197                     & (447) Chorozinho                     \\ \cline{1-2} \cline{4-5} 
\end{tabular}
\end{table}

==> table3.tex <==
\begin{table}[!t]
\centering
\caption{Results of the regression model showing estimates of the average marginal effect of the local economic complexity index with neighbors’ terms.}
\label{Table3}
    \begin{tabular}{lcccccccc}
    & \multicolumn{8}{c}{GDP growth, $g^t$}   \\ \hline
     & (1)  & (2)   & (3)   & (4)   & (5)   & (6)   & (7)   & (8)   \\ \hline
    IndECI     && & \begin{tabular}[c]{@{}l@{}}0.0987$^{***}$\\ (0.0198)\end{tabular}  & & \begin{tabular}[c]{@{}l@{}}0.0427$^{***}$\\ (0.0147)\end{tabular}  &  & & \\
    $\langle \text{IndECI} \rangle_N$ && & & \begin{tabular}[c]{@{}l@{}}0.1526$^{***}$\\ (0.0173)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.1056$^{***}$\\ (0.0147)\end{tabular}  & & & \\
    ECI  && & & & & \begin{tabular}[c]{@{}l@{}}0.0041\\ (0.0092)\end{tabular}     & & \begin{tabular}[c]{@{}l@{}}0.0044\\ (0.0071)\end{tabular}     \\
    $\langle \text{ECI} \rangle_N$    && & & & & & \begin{tabular}[c]{@{}l@{}}0.1330$^{***}$\\ (0.0164)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.1199$^{***}$\\ (0.0157)\end{tabular}  \\
    log $y$    && \begin{tabular}[c]{@{}l@{}}-0.4789$^{***}$\\ (0.0501)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.4182$^{***}$\\ (0.0369)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.3771$^{***}$\\ (0.0322)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.3254$^{***}$\\ (0.0266)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.4406$^{***}$\\ (0.0434)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.3593$^{***}$\\ (0.0337)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.3357$^{***}$\\ (0.0313)\end{tabular} \\
    log $N$    && \begin{tabular}[c]{@{}l@{}}-0.2672$^{***}$\\ (0.0702)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.2140$^{***}$\\ (0.5059)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.2025$^{***}$\\ (0.0504)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.1299$^{***}$\\ (0.0339)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.2271$^{***}$\\ (0.0598)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.2234$^{***}$\\ (0.0565)\end{tabular} & \begin{tabular}[c]{@{}l@{}}-0.2020$^{***}$\\ (0.0502)\end{tabular} \\
    $g^{t-1}$  & \begin{tabular}[c]{@{}l@{}}0.6393$^{***}$\\ (0.0320)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.3663$^{***}$\\ (0.0450)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.4113$^{***}$\\ (0.0365)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.4062$^{***}$\\ (0.0333)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.4447$^{***}$\\ (0.0301)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.3947$^{***}$\\ (0.0387)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.4151$^{***}$\\ (0.0319)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}0.4312$^{***}$\\ (0.0302)\end{tabular}  \\
    Constant   & \begin{tabular}[c]{@{}l@{}}0.0931$^{***}$\\ (0.0063)\end{tabular} & \begin{tabular}[c]{@{}l@{}}7.7413$^{***}$\\ (1.0896)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}6.5252$^{***}$\\ (0.7819)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}5.9851$^{***}$\\ (0.739)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}4.6335$^{***}$\\ (0.5153)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}6.9039\\ (0.9141)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}6.4831$^{***}$\\ (0.8511)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}5.9746$^{***}$\\ (0.7619)\end{tabular}  \\ \hline
    Fixed Effects \\
    Micro-region    & Yes  & Yes   & Yes   & Yes   & Yes   & Yes   & Yes   & Yes   \\
    Year  & Yes  & Yes   & Yes   & Yes   & Yes   & Yes   & Yes   & Yes   \\ \hline
    AB test    & \checkmark    & \checkmark     & \checkmark     & \checkmark     & \checkmark     & \checkmark     & \checkmark     & \checkmark     \\
    Sargan Test& \checkmark    & \checkmark     & \checkmark     & \checkmark     & \checkmark     & \checkmark     & \checkmark     & \checkmark     \\ \hline
    Observations   &5773&5773&5773&5773&5773&5773&5773&5773\\ \hline
    \end{tabular}
\end{table}
